The Quest for the Golden Activation Function

Deep Neural Networks have been shown to be beneficial for a variety of tasks, in particular allowing for end-to-end learning and reducing the requirement for manual design decisions. However, still many parameters have to be chosen in advance, also raising the need to optimize them. One important, but often ignored system parameter is the selection of a proper activation function. Thus, in this paper we target to demonstrate the importance of activation functions in general and show that for different tasks different activation functions might be meaningful. To avoid the manual design or selection of activation functions, we build on the idea of genetic algorithms to learn the best activation function for a given task. In addition, we introduce two new activation functions, ELiSH and HardELiSH, which can easily be incorporated in our framework. In this way, we demonstrate for three different image classification benchmarks that different activation functions are learned, also showing improved results compared to typically used baselines.

==> AF-learning_old.tex <==
\section{Learning of Combined Activation Functions}
\subsection{Genetic Algorithm}



In the proposed GA, an individual represents a piece-wise activation function as shown in \cref{fig:individual}. 
Please look at \cref{alg:ga} again. 
Initially, we generate a population of random activation functions; please see \cref{alg:ga:pop:init}. 
Next in \cref{alg:ga:fitness:init}, the fitness of each individual is determined by train and test performance of DNN. 
Indeed, DNN applies an individual as its activation function. 
Later in \cref{alg:ga:select}, we select a set of parent activation functions based on their fitness for breeding. 
To generate new activation functions, we apply a new crossover operator that we define later in the next subsection. 
Similarly, we update our population with the set of parents and bred offsprings and continue to the next generation.

\begin{figure}
\centering
\begin{tikzpicture}[scale=4/5, transform shape]
    \draw (0,0) rectangle node{activation left} (2.5,0.75);
    \draw (2.5,0) rectangle node{activation right} (5,0.75);
    \draw[decoration={brace},decorate](0,1)--node[blue,above=0.1]{Activation function} (5,1);
    %\draw[decoration={brace,mirror},decorate](0,-1) -- node[red,below=0.1] {Individual} (5,-1);
    \draw[decoration={brace,mirror},decorate](0,-0.25) -- node[blue,below=0.1] {Gene} (2.5,-0.25);
\end{tikzpicture}
\caption{An individual in the population of our Genetic Algorithm.}\label{fig:individual}
\end{figure}


\subsection{Crossover Operators}
We propose two different crossover operators namely ``Inheritance'' and ``Hybrid''. The latter operator combines parents' activation functions by means of mathematical operators. While applying the crossover operator we stochastically choose between Inheritance and Hybrid as shown in \cref{alg:method:crossover}.

\begin{algorithm}
    \caption{} \label{alg:method:crossover}
    \begin{algorithmic}[1]
    \Procedure{Crossover}{mom, dad}
    \State{$c$ $\gets$ toss a coin}
    \If{$c$ is heads}
        \State{\Return \textsc{Inheritance}(mom, dad)}
    \Else
        \State{\Return \textsc{Hybrid}(mom, dad)}
    \EndIf
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

\subsubsection{Inheritance.}
This operator is a one point crossover as described in preliminaries with only one difference. That is, its cutoff point is predetermined. The first (second) offspring inherits its left activation function from the mom (dad), and its right activation function from the dad (mom); please see \cref{fig:crossover:1}.

\begin{figure}
\centering
\begin{subfigure}{0.45\textwidth}
\centering
\begin{tikzpicture}[scale=4/5, transform shape]
    \draw (0,0) rectangle node{mom's left} (2,0.75);
    \draw (2,0) rectangle node{dad's right} (4,0.75);
    %\draw[decoration={brace},decorate](0,1)--node[blue,above=0.1]{Activation function} (4,1);
    %\draw[decoration={brace,mirror},decorate](0,-0.25) -- node[blue,below=0.1] {Gene} (2,-0.25);
\end{tikzpicture}
\caption{Offspring 1}\label{fig:crossover:1:child1}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\centering
\begin{tikzpicture}[scale=4/5, transform shape]
    \draw (0,0) rectangle node{dad's left} (2,0.75);
    \draw (2,0) rectangle node{mom's right} (4,0.75);
    %\draw[decoration={brace},decorate](0,1)--node[blue,above=0.1]{Activation function} (4,1);
    %\draw[decoration={brace,mirror},decorate](0,-0.25) -- node[blue,below=0.1] {Gene} (2,-0.25);
\end{tikzpicture}
\caption{Offspring 2}\label{fig:crossover:1:child2}
\end{subfigure}
\caption{Inheritance Crossover}\label{fig:crossover:1}
\end{figure}

\subsubsection{Hybrid Crossover.}
Hybrid crossover operator is proposed to combine activation functions. The cutoff point is fixed like Inheritance crossover. 
Using a randomly selected mathematical operator, the first (second) offspring combines mom's and dad's (dad's and mom's) left activation and takes it as its own left activation. 
Subsequently, the first (second) offspring's right activation function is a combination of mom's and dad's (dad's and mom's) right activation; see~\cref{fig:crossover:2}.


\begin{figure}
\centering
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}[scale=4/5, transform shape]
    \draw (0,0) rectangle node{$op_1$, mom's left, dad's left} (5,0.75);
    \draw (5,0) rectangle node{$op_2$, mom's right, dad's right} (10,0.75);
    %\draw[decoration={brace},decorate](0,1)--node[blue,above=0.1]{Activation function} (10,1);
    %\draw[decoration={brace,mirror},decorate](0,-0.25) -- node[blue,below=0.1] {Gene} (5,-0.25);
\end{tikzpicture}
\caption{Offspring 1}\label{fig:crossover:2:child1}
\end{subfigure}
\\\vspace{0.5cm}
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}[scale=4/5, transform shape]
    \draw (0,0) rectangle node{$op_1$, dad's left, mom's left} (5,0.75);
    \draw (5,0) rectangle node{$op_2$, dad's right, mom's right} (10,0.75);
    %\draw[decoration={brace},decorate](0,1)--node[blue,above=0.1]{Activation function} (10,1);
    %\draw[decoration={brace,mirror},decorate](0,-0.25) -- node[blue,below=0.1] {Gene} (5,-0.25);
\end{tikzpicture}
\caption{Offspring 2}\label{fig:crossover:2:child2}
\end{subfigure}
\caption{Hybrid crossover operator, where $op_1$ and $op_2$ are randomly selected from $\{+~,~-~,~*~,~/~,~\caret~,~\min,~\max,~f\circ g \}$.}\label{fig:crossover:2}
\end{figure}

\subsection{Mutate Operator}
The mutation operator randomly chooses a gene and then replaces it with a randomly selected predefined activation function; see \cref{fig:mutation}. In fact, this operator helps GA to keep exploring the search space for new activation functions.
\begin{figure}
\centering
\begin{tikzpicture}[scale=4/5, transform shape]
    \draw (0,0) rectangle node (A){mom's left} (2,0.75);
    \node [left=1cm of A] (B) {\begin{tabular}{c}Selected Activation:\\\textcolor{blue}{\relu}\end{tabular}};
    \draw (2,0) rectangle node{dad's right} (4,0.75);
    \draw [decoration={brace,mirror},decorate](0,-0.25) -- node[blue,below=0.1] {Selected Gene} (2,-0.25);
    \draw [->] (B) -- (A);
\end{tikzpicture}
\caption{A mutation operator}\label{fig:mutation}
\end{figure}

\subsection{Evaluating an Activation Function}
The Hybrid crossover operator results in a hybrid activation function that we evaluate by parsing according to the following grammar:
\begin{align}
    expr :=& f~|~operation,~epxr,~expr \notag  \\
    operation :=& +~| - | \times |~/~|\caret| \min | \max | ~f\circ g \notag \\
    f :=&~\elish~|~\hardelish~|~\swish~|~\relu~|~\elu~|~\selu~|~\sigmoid~|~\hardsigmoid~|
    \notag\\
    &~\sinus~|~\softplus~|~\linear~|
    \label{eq:function_list}
\end{align}
where $f$ represents the set of candidate solutions. One can easily extend the list of supported $operations$ and candidate solutions $f$.

\begin{example}
An example activation function generated by Hybrid crossover is:
\[
    (\max:(+:(\min:\elu:\relu):\swish):(\times:\elu:\linear))\;.
\]
\noindent Using \eqref{eq:function_list}, we parse above activation function as shown in \cref{fig:parsetree} which gives the following infix expression:
\[
    \max(\min(\elu,\relu)+\swish, (\elu \times \linear))\;.
\]

\begin{figure}
    \centering
    \begin{tikzpicture}[transform shape,
    ->,>=stealth',level/.style={sibling distance = 3cm/#1,level distance = 1cm}] 
    \node  {max}
        child{ node {$+$}
                child{ node {min} 
                        child{node {\elu}}
                        child{node {\relu}}}
                child{ node {\swish } } }
        child{ node {$\times$}
                child{ node {\elu}}
                child{ node {\linear}}};
    \end{tikzpicture}
\caption{An example of a parse tree} \label{fig:parsetree}
\end{figure}
\end{example}

\subsection{Implementation Details}
\label{sec:exp-setup}

\petermk{The following paragraph is not clear at all. In particular, it stays unclear how it is related to the appraoch described in Sec.4. Maybe, this discusion should be moved to the previous section, to make more apparent how the implementation and the technical description are related to each other?\mb{it is modified}}

Our implementation builds  based on DeepEvolve framework\footnote{\url{https://github.com/jliphard/DeepEvolve}}, a neuro-evolution framework to explore the optimal deep neural network topology for a given task. Our idea is differ from DeepEvolve in that the search space includes various hyper parameters such as the number of layers, the number of neurons and so on. In our case, the DNN topology is fixed for each task and the search space is defined based on the activation functions. Moreover, We proposed two new crossover operators.
 

==> defs.tex <==


% Uncomment for the submitted version !!!
%\renewcommand{\peterrmk}[1]{{{\color{BrightRoyalPurple}{}}}}
%\renewcommand{\mb}[1]{}

%% \newcommand{\peter}[1]{{{\color{RoyalPurple}{#1}}}}
%% \newcommand{\peterc}[2]{{{\color{RoyalPurple}{#1}}}}
%% \newcommand{\peterrmk}[1]{{{\color{RoyalPurple}{\bf #1}}}}


==> preliminaries.tex <==
\section{Preliminaries}

\petermk{I am thinking on skipping this section, in particular if the new AFs are introduce seperately. There is much redundent information, thus the relevant information can be moved to the next section.}

\subsection{Genetic Algorithm}
Genetic Algorithm (GA) is a population-based metaheuristic. Metaheuristic is indeed the primary sub-field of stochastic optimization \cite{DeJong2006a}. In General, we apply metaheuristics to ``I know it when I see it.'' problems. Which means we are given a broad set of candidate solution, but we do not know how the optimal solution might be or do not know how to approach it principally \cite{Luke2009Metaheuristics}. Please see \cite{PB10}, to find out more about the reasons for employing population-based approach. The role of the population is the representation of possible candidate solutions. In a nutshell, the candidate solutions in population-based approaches affect each other concerning how they reach global optima. 

\Cref{alg:ga} gives a comprehensive pseudocode of GA. Initially, we generate a population of random solutions; please see \cref{alg:ga:pop:init}. Each solution in this population is called an individual. Next in \cref{alg:ga:fitness:init}, we evaluate the fitness of all individuals in the population. Later in \cref{alg:ga:select}, we select a set of parent solutions based on their fitness for breeding. Subsequently, we apply breeding operators on pairs of individuals in ``parents'' to generate new pairs of offsprings; please see \crefrange{alg:ga:breeding:start}{alg:ga:breeding:end}. Eventually in \cref{alg:ga:pop:update}, we update our population with the set of parents and bred offsprings. We loop over \crefrange{alg:ga:generation:start}{alg:ga:generation:end} up to the satisfaction of the termination condition. Each iteration of this loop is called a generation in GA related literature.

%The basic Genetic algorithms is shown in following pseudo-code.
\scalebox{0.7}{
\begin{minipage}{.65\linewidth}
\begin{algorithm}[H]
    \caption{Pseudocode of Genetic Algorithm} \label{alg:ga}
    \begin{algorithmic}[1]
     \Procedure{GeneticAlgorithm}{population-size}
     \State{population $\gets \emptyset$}
     \State{population $\gets$ \textsc{Initialize}(population-size)}
     \label{alg:ga:pop:init}
     \State{\textsc{Evaluate}(population)}
     \label{alg:ga:fitness:init}
     \Repeat
     \label{alg:ga:generation:start}
        \State{children $\gets \emptyset$}
        \State{parents $\gets$ \textsc{Select}(population)}
        \label{alg:ga:select}
        \For{$\langle$mom, dad$\rangle \in$ parents $\times$ parents}\label{alg:ga:breeding:start}
            \State{offsprings $\gets$ \textsc{Crossover}(mom, dad)}
            \For{offspring $\in$ offsprings}
                \State{offspring $\gets$ \textsc{Mutate}(offspring)}
            \EndFor
            \State{\textsc{Evaluate}(offsprings)}
            \label{alg:ga:fitness:offsprings}
            \State{children $\gets$ children $\cup$ offsprings}
        \EndFor\label{alg:ga:breeding:end}
        \State{population $\gets$ parents $\cup$ children}
        \label{alg:ga:pop:update}
    \Until{termination condition}
    \label{alg:ga:generation:end}
    \State{\Return population}
    \EndProcedure
    \end{algorithmic}
\end{algorithm}
\end{minipage}
}
\scalebox{0.7}{
\begin{minipage}{.76\linewidth}
\begin{algorithm}[H]
    \caption{Pseudocode of One Point Crossover \cite{Luke2009Metaheuristics}} \label{alg:ga:onepoint-crossover}
    \begin{algorithmic}[1]
     \Procedure{Crossover}{Mom,Dad}
     \State{$\vec{v} \gets$  a vector of Mom's genes to be crossed over}
     \State{$\overrightarrow{w} \gets$  a vector of Dad's genes to be crossed over}
     \State{$n \gets |\vec{v}|$} \Comment{number of genes in $\vec{v} \text{ and } \vec{w}$}
     \item[]
     \State{$c$ $\gets$ random integer chosen uniformly from 1 to $n$ inclusive}
     \If{$c\neq1$}
         \For{$i$ from $c$ to $n$ }
           \State{ Swap the values of genes {$v_i$} and {$w_i$}}
         \EndFor 
    \EndIf     
    \State{\Return {$\vec{v}$} and {$\vec{w}$} }
    \EndProcedure
    \end{algorithmic}
\end{algorithm}
\end{minipage}
}

\subsection{Crossover}
Crossover or Recombination is a stochastic operator. The operator exchanges information between parents to form a new offspring. The crossover is unable to provide new gen value for the offspring. However, it is enabled to increases the exploratory power of GA.  Researchers defined a variety of Crossover operators; for instance, one point crossover wherein, the operator selects a random point at which parental genes are swapped.

\subsection{Mutation}
Mutation is a stochastic operator that helps to increase the diversity of the population. It randomly chooses one or a number of genes in an offspring and changes them. This act leads to a mutated offspring. There are different type of mutation operators. For example, in uniform mutation, the operator changes the value of chosen gene with uniform random value. It is used in case of real and integer representation.  





==> trash.tex <==
\petermk{TRASH TRASH TRASH -- blow this line -- TRASH TRASH TRASH}


\subsection{Benchmark Datasets}
\label{sec:benchmarks}
 
 We run experiments on three different object classifications benchmarks (\ie CIFAR-10 \cite{Krizhevsky09a}, CIFAR-100 \cite{Krizhevsky09a}, and Tiny ImageNet\footnote{\url{https://tiny-imagenet.herokuapp.com/}}), differing in number of classes, number of samples, and complexity:
 
\vspace{-0.25cm}
\begin{description}[style=unboxed,leftmargin=0cm]

\item[CIFAR-10] consists $60,000$ $32 \times 32$ color images describing $10$ classes. For each class $5,000$ training and $1,000$ test samples are provided, respectively.

\vspace{0.15cm}

\item[CIFAR-100] also consists of $60,000$ $32 \times 32$ color images, however, the number of classes and samples per class differ: The data set consists of  $100$ classes, however, for each class only $500$ training and $100$ test samples are provided, respectively.
\vspace{0.15cm}

\item[Tiny ImageNet] is based on the ILSVRC2016 dataset\footnote{\url{http://image-net.org/challenges/LSVRC/2016/}}, where a subset of images was selected and cropped/re-sized. 
 The dataset consists of $120,000$ $64\times64$ color images, organized in $200$ classes, where for each class $500$ training, $50$ validation, and $50$ test images are given.

\end{description}




Deep Neural Networks (DNNs) \cite{pmroth:schmidhuber15,pmroth:goodfellow16,pmroth:lecun15} have recently become very popular and are now widely applied for different applications including image segmentation \cite{pmroth:ronneberger15, Badrinarayanan15}, image classification \cite{He:2015:DDR:2919332.2919814, pmroth:krishevski12} or medical image analysis \cite{pmroth:liu17, pmroth:esteva17, pmroth:Litjens17}. In general, DNNs are inspired by the human brain, which is a complex network made up of neurons connected via synapses. However, in contrast to biological neural networks, the neurons are organized in multiple layers with specific connections and directions of information propagation, allowing for learning complex functions. The most prominent approach are Convolutional Neural Networks (CNNs) \cite{pmroth:lecun98}, which are structured in a series of different layers, \ie convolutional layers, pooling layers, and fully connected layers. In this way, complex target functions can be learned, however, also the estimation of the system parameters is getting very complicated.

Therefore, there have many strategies been developed to make neural network training more efficient and more stable. For instance, to avoid that the optimization process gets stuck in a local optimum, the initialization of trainable parameters is of high relevance. Thus, there has been a considerable interest in different initialization techniques for trainable parameters (\eg \cite{Sutskever:2013:IIM:3042817.3043064,DBLP:journals/corr/Sussillo14,Mishkin2015AllYN}). Another well known and well studied problem is data normalization, which influences both the quality of the results and the stability. To this end, there was recently a considerable interest in normalization techniques to steer the optimization process (\eg \cite{laurent16,DBLP:journals/corr/BaKH16}). As both problems are of relevance, initialization and normalization techniques are often applied together and their interaction to one-another is studied (see \eg \cite{DBLP:conf/nips/KlambauerUMH17}).


%using an Adam optimizer, , t, \petermk{(vs. decay??!!)} \mb{decay rates are different for VGG16 and Resnet56; I will get to it by tomorrow noon}, and the batch size is set to $32$. The numbers of epochs are 120 and 200 for Renset56 and VGG16 \cite{Simonyan15}, respectively.


\comment{


\mbtext{Even though a larger population size helps GA to better explore the search space, it is usually chosen empirically and based on the nature of task. Many works related to evolve DNN topology (\eg \cite{DBLP:journals/corr/RealMSSSLK17}) consider population size around $100$ where many hyper-parameters are involved.} 


\petermk{Is there any plausible argument for 8 generations? Are there any differences visible from generation to generation: are the results changing dramatically, are the functions are changing?}
\mb{I choose 8 generations because 
1. I did it empirically; as each generation add to the complexity of candidate AFs after the 8th generation the training will increase drastically for deep networks.
2. and again we do not have enough computational power to run experiments for that.
3. In the cited paper you can also see the population size and training epochs are chosen empirically because it is difficult to find a theoretical justification for it.
}

% more completely. But usually we have a limited computational resources that restricts the population size. So, empirically and based on the previous works  we found that the population of size 40 can be a right choice. The population evolves over eight generations. 

}
% The learning rate is decay and Adam is considered as an optimizer.

%The VGG16 is implemented by Keras library and Tensorflow. 

%Early stopping is used to reduce the training time during an evolution.


%%We evaluate the top activation functions on Resnet56 architecture and VGG16 to find out how much they are robust to the large models. The learning rate and batch size are same as before. The learning rate is decay and Adam is considered as an optimizer.  The weights are initialized by  \texttt{He-Normal}. The neural network applies a \func{softmax} activation function in their output layer and is trained by minimizing the average cross-entropy on the training data. The number of epochs are 120 and 200 for Renset56 and VGG16 \cite{Simonyan15} respectively. The VGG16 is implemented by Keras library and Tensorflow. 


 %%In the course of evolution, a . Which are trained for seven epochs using the Tensorflow library. The learning rate is $1e-3$ and the batch size is set to 32 that are same for all experiments throughout the paper. Early stopping is used to reduce the training time during an evolution.



\subsection{Activation Functions}
\subsubsection{Squashing}
The advances in neuroscience encouraged to define nonlinear functions like squashing functions. The most popular squashing functions are Sigmoid \cref{eq:Sigmoid} and hyperbolic tangent (\ie \func{Tanh}) \cref{eq:Tanh}. The remarkable characteristic of such activation functions is that the amplitude of function will be very small when input values goes beyond a certain range (\ie Saturation regions). Both activation functions are shown in Figure 2 and 3 respectively. 
\begin{figure}[h!]
  \centering
  \noindent
  \begin{minipage}{.35\linewidth}
    \input{figures/sigmoid.tex}
    
  \end{minipage}%
  \begin{minipage}{.45\linewidth}
    \begin{equation}
    \label{eq:Sigmoid}
       y(x) = \frac{1}{1+e^{-x}}
    \end{equation}
  \end{minipage}
  \caption{Sigmoid Function}
  \label{fun:sigmoid}
\end{figure}


As it shown in \Cref{fun:sigmoid},  \sigmoid~outputs are not zero-centered. It causes the successive layers in DNNs get input values which are all positive or all negative. Then updated weight during Backprobackagation will have same signs as input values. It conducive to oscillatory behaviour in dynamic of gradient and also make convergence too slow. In contrast, \tanh~speeds up the training  faster since it is symmetric around zero and the range of response (amplitude) is well-defined. As it illustrates in \Cref{fun:sigmoid}. In squashing functions, the first-order derivative of the function becomes close to zero when input values map to the saturated region which causes vanishing gradient problem during back propagation. It affected optimization convergence, and in some cases, the final trained network converges to a poor local minimum.

 
 \begin{figure}
  \centering
  \noindent
  \begin{minipage}{.35\linewidth}
%    \input{figures/tanh.tex}
    
  \end{minipage}%
  \begin{minipage}{.45\linewidth}
    \begin{equation}
    \label{eq:Tanh}
       y(x) = \frac{2}{1+e^{-2x}}-1
    \end{equation}
  \end{minipage}
  \caption{Tanh Function}
  \label{fun:Tanh}
\end{figure} 

%====================================================================
\subsubsection{Rectifier Linear Units}
Rectifier linear function \relu~is proposed to prevent a vanishing gradient problem since it has identity function in positive part. This activation function is anti-symmetric about $0$ and has a more gradual gradient than a \sigmoid~. As a result, it often leads to more robust optimization during DNN training. However, the error propagation will stop during optimization whenever the unit is not active, which is a potential disadvantage. Because, certain amount of bias gets propagated to the higher layers of the network. That changes the desirable range of updated weights. \Cref{fun:Relu} shows \relu. The function is mathematically given by \Cref{eq:Relu}.

\begin{figure}[h]
  \centering
  \noindent
  \begin{minipage}{.35\linewidth}
    \input{figures/Relu.tex}
    
  \end{minipage}%
  \begin{minipage}{.55\linewidth}
    \begin{equation}
    \label{eq:Relu}
       y(x) = \max(x,0)
    \end{equation}
  \end{minipage}
  \caption{ReLU Function}
  \label{fun:Relu}
\end{figure} 

%====================================================================================================


\subsubsection{Exponential Linear Unit}
Compare to \func{LReLU}, negative values in \elu~are smooth and saturate to smaller exponential values which help them to be more closer to zero mean unit activations. That eventually, speeds up learning process. However, Incompatibility with Batch-normalization is an undesirable characteristic of \elu~. \Cref{fun:ELU} shows the \elu~activation function. The \elu~is mathematically given by \Cref{eq:ELU}.

\begin{figure}[h!]
  \centering
  \noindent
  \begin{minipage}{.35\linewidth}
    \input{figures/ELU.tex}
    
  \end{minipage}%
  \begin{minipage}{.55\linewidth}
    \begin{equation}
    \label{eq:ELU}
     y(x)=
      \begin{cases}
      
        \alpha(e^x-1) & x< 0\\
        x & x \geq 0
      \end{cases}
    \end{equation}
  \end{minipage}
  \caption{ELU Function}
  \label{fun:ELU}
\end{figure} 

\subsubsection{ Scaled Exponential Linear Unit}
To embed Batch Normalization method (BN) inside the activation function a slight modification of \elu~called \selu~including scaling factors is proposed. The scaling factors are as follows; $\alpha=1.6732\sim$, $\lambda=1.0507\sim$. They are theoretically proven to these certain values. Slop ($\lambda$) defines larger than one to prevent the variance becomes too small in lower layer. \Cref{fun:SELU} shows the \selu~activation function. The function is mathematically given by \Cref{eq:SELU}.

\begin{figure}[h!]
  \centering
  \noindent
  \begin{minipage}{.35\linewidth}
    \input{figures/selu.tex}
    
  \end{minipage}%
  \begin{minipage}{.55\linewidth}
  
    \begin{equation}
      \label{eq:SELU}
      y(x)=
      \lambda\begin{cases}
        \alpha(e^x-1) & x< 0\\
        x & x \geq 0\\
      \end{cases}
    \end{equation}
     
  \end{minipage}
  \caption{SeLU Function}
  \label{fun:SELU}
\end{figure} 

\subsubsection{Swish}
Swish is multiplication of identity function and \sigmoid. The \sigmoid~part is multiplied by a scaling factor $\beta$ which is either a constant or a trainable parameter. Compare to \relu~, \func{Swish} has a non-monotonic behavior in negative part such that the behavior controls by $\beta$ values. \Cref{fun:Swish} shows \swish~function. The function is mathematically given by \Cref{eq:Swish}.
\begin{figure}[h!]
  \centering
  \noindent
  \begin{minipage}{.35\linewidth}
    \input{figures/swish.tex}
    
  \end{minipage}%
  \begin{minipage}{.55\linewidth}
    \begin{equation}
      \label{eq:Swish}
      y(x)=
         \frac{x}{1+e^{(-\beta x)}}
       \end{equation}
  \end{minipage}
  \caption{Swish Function}
  \label{fun:Swish}
\end{figure} 

\begin{figure}
\centering
\begin{subfigure}{0.49\textwidth}
	\centering
	\includegraphics[width=\textwidth,trim={1.0cm 0.4cm 1.0cm 0.9cm},clip]{figures/cifar10-result-ResNet56.eps}
	\caption{Accuracy}
	\label{fig:1a}		
\end{subfigure} \hfill
\begin{subfigure}{0.49\textwidth}
	\centering
	\includegraphics[width=\textwidth,trim={1.0cm 0.4cm 1.0cm 0.9cm},clip]{figures/cifar10-result-ResNet56-loss.eps}
	\caption{Loss}
	\label{fig:2a}		
\end{subfigure}
\caption{Performance of explored activation functions for Cifar10}
\end{figure}

{\frac{exp(-x)}{(1+exp(-x))^2}+x*1/(1+exp(-x))}
(exp(-x)/(1+exp(-x))^2)* (exp(x)-1)+exp(x)*1/(1+exp(-x))
 \begin{minipage}{.55\linewidth}
  
    \begin{align}
      \label{eq:elish}
      y(x\geq 0)&= \frac{x}{1+e^{-x}}\\
      y(x<0)&= \frac{e^x-1}{1+e^{-x}}
    \end{align}
     
  \end{minipage}
2.
&
93.07\%
&
$
y(x<0)= \hardelish  \text{ and } y(x\geq0)= \relu** Resnet-cifar10
$
\\
6.
&
92.76\%
&
$
y(x<0)= \hardelish  \text{ and } y(x\geq0)= \relu** VGG-cifar10
$
\\
8.
&
70,79\%
&
$
y(x<0) = \elish\text{ and } y(x\geq0)=\max(\linear,\sinus)-resnet cifar100
$
\\
5.
&
70.79\%
&
$
y(x<0) = \elish\text{ and } y(x\geq0)=\max(\linear+\sinus)
$
\\


Constructive means, that starting with a simple topology gradually the complexity is increase until an optimality criterion is satisfied. In contrast, destructive means the initial topology is complex and incrementally reduces the unnecessary neurons and layers in DNN. \petermk{... to be completed\mb{done}} In this way, \cite{8020002} proposed a constructive EA to generate DNN for pattern classification. \petermk{More details are needed here!} Similarly,
\cite{recurrentnode} applied the constructive strategy to evolve both recurrent nodes and RNN's architecture network. \petermk{I do not understand this sentence?}
%In this study, a layer is constructed by adding evolved recurrent node step by step; then, the layer is optimized using complex recurrent nodes that are evolving over generations. Finally, the evolved layers form an optimal topology.
In contrast, \cite{Hancock92pruningneural} applied a destructive strategy to prune the ANN, which aims at decreasing its complexity and improve its numerical stability.

%introduction
Initially, due to their universal approximation properties the research in this field was mostly concentrated on squashing functions such as \sigmoid and \tah  \cite{Hornik:1991:ACM:109691.109700}.
However, when training DNNs using such functions suffers from the vanishing gradient problem \cite{vanishing}.\mbtxt{ When the gradient of the objective function approaches zero very slowly, then gradient decent algorithm takes smaller steps towards the local minimum and more time to converge; this is vanishing gradient problem} \petermk{a half sentence missing here to explain this term!\mb{done}} To overcome this problem, various non-squashing functions were introduced \cite{} \petermk{at this points references might be missing}, where the most notable example is Rectified Linear Unit (\relu) \cite{Nair:2010:RLU:3104322.3104425}. In particular, as the derivative of positive inputs in \relu are one, the gradient cannot vanish. In contrast, as all negative values are mapped to zero, there is not information flow in DNNs for negative values. This problem is known as dying \relu. 

To overcome this problem, various generalizations of \relu such \func{Leaky} \relu \cite{Maas13rectifiernonlinearities} have been proposed. Negative values in \func{Leaky} \relu pushes means activation values towards zero. Similarly, (\elu) \cite{DBLP:journals/corr/ClevertUH15} is proposed which not only eliminates the bias shift in the succeeding layers. By returning a bounded exponential value for negative inputs, but also pushes the  mean activation value toward zero.

\petermk{also here more references might be needed}. However, \func{Leaky} \relu suffers from the problem that the deactivation state is not noise-robust. \petermk{What does this mean?} This problem can be avoided by Exponentiation Linear Unites (\elu) \cite{DBLP:journals/corr/ClevertUH15} , which additionally eliminate the bias shift in the succeeding layers. 
By returning a bounded exponential value for negative inputs, \elu is saturated at a predefined threshold and the mean activation value is pushed toward zero. \petermk{Is this true? This might be formulated in a better way?} Although, showing competitive results, \elu not backed by a very strong theory. A theoretically proven modification, Scaled Exponentiation Linear Unites (\selu) \cite{DBLP:conf/nips/KlambauerUMH17}, make DNN learning more robust. It fact, it is shown that the proposed self-normalizing network converges towards a normal distribution with zero mean and unit variance.

% To be removed, when comments are removed
\vspace{-0.25cm}
%
A different direction was pursued in \cite{Ramachandran18}, finally introducing the \swish activation function. Different search spaces are created by varying the number of core units used to construct the activation function, and an RNN is trained to search the state space for a novel activation function.
%The core units consist of various unary and binary functions.
The proposed approach shows competitive results for both shallow and deep neural networks. Recently, a theoretic proof for the claimed benefits haven been given in \cite{hayou18}.

% To be removed, when comments are removed
\vspace{-0.25cm}
%
In this way, existing approaches to estimate activation functions for DNN learning are lacking theoretical foundation, are based on complex theory, which is hard to understand in the context of practical applications, or are based on inefficient search schemes, which still require to manually set several parameters. To overcome these problems, we propose an approach based on ideas of Genetic Algorithms \cite{GA-intro}. In particular, building on neuro-evolutionary \cite{Neuro-intro}, starting from simple initial activation functions more and more complex functions can be obtained over time, which are better suited for a given task. In contrast, to brute-force search strategies, the search space is explored in more efficient way, drastically reducing the training effort. In addition, we propose to define piece-wise  functions, better representing the (theoretically) desired properties, which can be easily considered in the proposed framework. 

% To be removed, when comments are removed
\vspace{-0.25cm}
%
As second contribution, based on recent theoretical findings \cite{hayou18}, we introduce two new activation functions, namely, \elish and \hardelish, which have shown to be competitive compared to existing approaches as well as very useful within the proposed framework. To demonstrate the benefits of our learned  activation function, we applied our approach for three different object classification benchmark data sets, varying in size and complexity, using two different network architectures. The results clearly demonstrate that using the proposed approach better results can be obtained as well as that for different tasks different activation functions might be useful.

% To be removed, when comments are removed
\vspace{-0.25cm}
%
The reminder of the paper paper is structured as follows: First, in Sec.~\ref{sec:related}, we discuss the related work in the context of Genetic Algorithms for Neural Networks. Next, in Secs.~\ref{sec:elish}~and~\ref{sec:lcaf} we introduce our new activation functions and the proposed neuro-evolutionary learning of activation functions. Then, in Secs.~\ref{sec:results}, we give a detailed experimental evaluation of our approach and discuss the findings. Finally, in Sec.~\ref{sec:conclusion} we summarize and conclude our work.
 
 \pagebreak


%On the other hand theoretical proofs can be very complex  (\eg \cite{DBLP:conf/nips/KlambauerUMH17, hayou18}). Most recently, search based techniques emerged to automate trial-and-errors in designing activation functions \cite{Ramachandran18}, where the goal is to solve an optimization problem to find an activation function best suited for a given problem. As the search space, however, could be rather large, the approach is not very efficient and s
